Online certification of preference-based fairness for personalized recommender systems

Recommender systems are facing scrutiny because of their growing impact on the opportunities we have access to. Current audits for fairness are limited to coarse-grained parity assessments at the level of sensitive groups. We propose to audit for envy-freeness, a more granular criterion aligned with individual preferences: every user should prefer their recommendations to those of other users. Since auditing for envy requires to estimate the preferences of users beyond their existing recommendations, we cast the audit as a new pure exploration problem in multi-armed bandits. We propose a sample-efficient algorithm with theoretical guarantees that it does not deteriorate user experience. We also study the trade-offs achieved on real-world recommendation datasets.

==> sections/appendices/groups.tex <==
\section{Groups in practice}\label{app:howtogroup}

Here we describe a favorable property of homogeneous groups and its implication for constructing groups in practice.

When policies in groups are homogeneous, then the average group policy and the transported policy are similar, so $\epsilon$-envy-freeness translates to $\epsilon'$-group envy-freeness for average group policies as well, with $\epsilon'\approx \epsilon$. More interestingly, when we have prior knowledge that users in all groups have homogeneous preferences and homogeneous policies, the reciprocal of Proposition \ref{prop:transport} from Sec. \ref{sec:GEF} holds for both average and transported policies:
\begin{proposition}\label{prop:GEFtoEF}
Let $\epsilon, \tilde{\epsilon}>0$, and assume that for all groups $\gr\in\intint{\ngroups}$ and all pairs of users $\user, \otheruser$ in the same group $\group_\gr$, we have
\begin{align*}
    &~\sup_{\ctx\in\ctxS} \norm{\pi^\user(.|\ctx) - \pi^\otheruser(.|\ctx)}_1 \leq \tilde{\epsilon}
    \text{~~and~~} \\
    &\sup_{\ctx\in\ctxS} \norm{\exprew^\user(.|\ctx) - \exprew^\otheruser(.|\ctx)}_1 \leq \tilde{\epsilon}.
\end{align*}
Then, with either average group policies or transported group policies, $\epsilon$-group envy-freeness implies $(\epsilon+4\tilde{\epsilon})$-envy-freeness.
\end{proposition}
The result is natural since when all groups have users with homogeneous preferences and policies, groups and users are a similar entity as far as the assessment of envy-freeness is concerned. The proof is straightforward and omitted. The interest of this remark lies in a better understanding of how to construct groups in practice, since homogeneity in policies and preferences impact how much a certificate of $\epsilon$-group envy-freeness should be interpreted as a certificate of $\epsilon'$-envy-freeness with $\epsilon'\approx \epsilon$. 

%We now briefly mention some possible ideas to construct groups $\group_\gr$ in practice. 

In the favorable case where we have strong prior knowledge on user preferences, building groups by clustering by user preferences allows the conditions of Proposition \ref{prop:GEFtoEF} to hold (assuming the system meets the minimal requirement of similar policies given similar preferences). The number of users in each cluster controls the trade-off between the strength of the guarantee (in terms of $\epsilon+4\tilde{\epsilon}$ of Prop. \ref{prop:GEFtoEF}\footnote{$\tilde{\epsilon}$ is typically larger as soon as groups contain more users.}) and the number of required exploration steps per user. In that case, the certification of envy-freeness aims at certifying that preferences are properly represented in the recommendations.
%(since the prior knowledge is about similarity in preferences between users, which is different from the knowledge of the preferences themselves).

In many cases, however, the auditor does not have prior knowledge on user preferences. An audit for group envy-freeness in this case will likely only be able to detect envy when some groups receive systematically worse recommendations than other groups. In the literature on fairness in machine learning, groups are most often defined by identity of sensitive attributes such as gender, ethnicity, age \cite{barocas2016big}, as well as intersections of them \cite{kearns2018preventing}, because these are dimensions of frequent systematic undesirable bias. Thus, groups that only differ by a value of these attributes should be compared.

%In addition to sensitive attributes, in many applications, additional features define finer grained groups while restricting comparability. An important one is the notion of eligibility of users to recommendations. When recommending accommodations for instance, most items should not be shown to some users because they don't match in terms of predefined search criteria such as desired location or price, irrespective of finer-grained user preferences. Groups created by crossing eligibility with sensitive attributes would create finer grained and more homogeneous groups, and using eligibility to the same recommendations as a constraint for comparability allows to reduce the number of comparable groups (and thus the sample complexity) without losing in relevance. Of course, depending on the context, additional features could be helpful to create finer-grained groups depending on the allowed exploration budget. %\virginie{maybe \cite{ilvento2020multi} here}


==> sections/appendices/other_datasets.tex <==
\section{Additional experiments}\label{app:add-xps}

We present a batch of experiments with different settings than the main one presented in Section \ref{sec:exps}. Since all results are qualitatively similar, we did not include them in the core paper. The goal is to confirm the following claim: the sparsity of the training set only affects the quality of the recommender system, and not the auditing process. 

Using the same protocol, we repeated the experiments from Section \ref{sec:exps} using 1) subsampled training sets from MovieLens-1M with different levels of sparsity and 2) an additional ratings dataset, Google Local ratings\footnote{Available at \url{https://cseweb.ucsd.edu/~jmcauley/datasets.html}}. 

Precisely, to study the effect of sparsity, we subsampled training sets with $10\%$ and $5\%$ of the MovieLens ``ground truth'' ratings (obtained with matrix completion). As in our main experiments, these training sets are given as input to the FunkSVD algorithm, and the recommender system uses a softmax policy over predicted ratings. We remind that in Sec. \ref{sec:exps}, the same protocole was used with a training set made of $20\%$ of the ratings.

Then, to compare our results on MovieLens with another dataset, we use the Google Local ratings dataset from \cite{he2017translation}. It includes reviews and ratings from 11,4M users about 3,1M businesses. As in \cite{patro2020fairrec}, we restrict the dataset to users and businesses located in New York and with at least 10 reviews. We draw a random sample of 2,000 users among the remaining ones. With the same protocole as for MovieLens, we generate ``ground truth'' ratings for each user-item pair with standard matrix completion. This results in a full rating matrix with 2,000 users and 855 items. As before, we simulate a recommender system by training Funk-SVD on a subsample of $20\%$ of the ratings, and using a softmax policy over predicted ratings. In the absence of demographic attributes, we focus on individual envy-freeness.

For the experiments on envy from mispecification (as in Sec. \ref{sec:exp-envy}), Figures \ref{fig:mispec-0.05}, \ref{fig:mispec-0.10}, \ref{fig:mispec-glr} show that the degree of envy varies similarly w.r.t. the number of latent factors across experimental settings. The only difference is the amplitude of envy.

Then, we evaluate the auditing algorithm (as in Sec. \ref{sec:exp-ocef}) on each of these environments, and observe that the performance of \banditalg is not affected. Fig. \ref{fig:ocef-sparse_alpha}, \ref{fig:ocef-sparse_delta} show that the results are qualitatively similar when recommendations are generated from sparser rating matrices extracted from MovieLens.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{ocef/figs/new_exps/mispec_softmax_100_sparsity_5_nsims4.png}
    \caption{Model mispecification on MovieLens with Softmax policy, trained on $5\%$ of the ratings. Groups are defined by age-occupation. \label{fig:mispec-0.05}}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{ocef/figs/new_exps/mispec_softmax_100_sparsity_10_nsims5.png}
    \caption{Model mispecification on MovieLens with Softmax policy, trained on $10\%$ of the ratings. Groups are defined by age-occupation. \label{fig:mispec-0.10}}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{ocef/figs/new_exps/GoogleLocal_mispec_softmax_100_sparsity_20_nsims5.png}
    \caption{Model mispecification on Google Local with Softmax policy, trained on $20\%$ of the ratings. \label{fig:mispec-glr}}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{ocef/figs/new_exps/all_vs_alpha_movielens_sparsity_5e-2.png}
    \caption{Scaling w.r.t. $\alpha$ on MovieLens experiments, with a sparsity level of $5\%$. \label{fig:ocef-sparse_alpha}}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{ocef/figs/new_exps/all_vs_delta_movielens_sparsity_5e-2.png}
    \caption{Scaling w.r.t. $\delta$ on MovieLens experiments, with a sparsity level of $5\%$. \label{fig:ocef-sparse_delta}}
\end{figure}

==> sections/appendices/pull_arm.tex <==
\section{The PULL-ARM routine}\label{app:pull-arm}

The PULL-ARM routine used in Alg.~\ref{alg:bandit-sync} is described in Alg.~\ref{alg:pull-sync}.

\begin{algorithm}[t]
\caption{\texttt{PULL-ARM} using transported policies (line 4).\label{alg:pull-sync}}
 \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
 \SetKwProg{DoParallel}{in parallel}{ do}{end}
 
 \Input{arm $\grarm$, timestep $t$, user group $\group$}
 \Output{Observed group reward $r_t$}
  \ForEach(\tcp*[f]{in parallel}){user $\user \in \group$}{
    Observe context $\ctx^\user_t \sim q^\user$\;
    \lIf{k=0}{$n = m$\tcp*[f]{pull baseline}}
    \lElse{Sample ``other user'' $\otheruser\sim\tilde{\gamma}^*_{m,.}$\tcp*[f]{Def. \ref{dfn:transportedpol}}}
    Show $\act_t^\user \sim \pi^n(.|\ctx^\user_t)$ and observe $\rew^\user_t\sim \nu^\user(\act_t^\user| \ctx^\user_t))$\;
    }
  \Return $\rew_t = \frac{1}{\card{\group}}\sum_{\user\in\group} \rew^\user_t $\;
\end{algorithm}

